The Gaia-ESO Survey: Calibrating the lithium-age relation with open clusters and associations. II. Expanded cluster sample and final membership selection

The Li abundance observed in pre-main sequence and main sequence late-type stars is strongly age-dependent, but also shows a complex pattern depending on several parameters, such as rotation, chromospheric activity and metallicity. The best way to calibrate these effects, with the aim of studying Li as an age indicator for FGK stars, is to calibrate coeval groups of stars, such as open clusters (OCs) and associations. We present a considerable target sample of 42 OCs and associations, ranging from 1 Myr to 5 Gyr, observed within the Gaia-ESO survey (GES), and using the latest data provided by GES iDR6 and the most recent release of Gaia that was then available, EDR3. As part of this study, we update and improve the membership analysis for all 20 OCs presented in our previous article. We perform detailed membership analyses for all target clusters to identify likely candidates, using all available parameters provided by GES and based on numerous criteria: from radial velocity distributions, to the astrometry and photometry provided by Gaia, to gravity indicators, [Fe/H] metallicity, and Li content. We obtain updated lists of cluster members for the whole target sample, as well as a selection of Li-rich giant contaminants obtained as an additional result of the membership process. Each selection of cluster candidates was thoroughly contrasted with numerous existing membership studies using data from Gaia to ensure the most robust results. These final cluster selections will be used in the third and last paper of this series, which reports the results of a comparative study characterising the observable Li dispersion in each cluster and analysing its dependence on several parameters, allowing us to calibrate a Li-age relation and obtain a series of empirical Li envelopes for key ages in our sample.

==> Caption/CHANGELOG <==
Changes made in the caption package bundle
==========================================

Please note that this document does not reflect bugfix-releases (which are marked with a letter after the version number, for example v3.4m), and that the dates given are the dates of the release w/o bugfixes.

If you are interested in a complete changelog -- including bugfixes -- process the dtx files with \RecordChanges and \PrintChanges.


caption package
---------------

v1.0 (1994/10/27)
- 1st published version

v1.1 (1994/11/03)
- New option `centerlast'

v1.2 (1994/11/28)
- Support of the `float' package added

v1.3 (1995/01/09)
- Support of \captionlabelfont in subcaptions added

v1.4 (1995/01/30)
- New option `nooneline'

v2.0 (caption2, 1995/10/09)
- New experimental version with many new commands and features
- Support of the `longtable' package added

v2.1 (caption2, 2002/02/26)
- Adapted to version 2.1 of the subfigure package
- New options for interaction with other packages (float,...)
- New command \normalcaptionparams
- New commands \captionof and \captionof*
- New ifs \ifcaptionlabel and \ifignoreLTcapwidth
- \realcaptionwidth renamed to \captionlinewidth

v2.2 (caption2, 2007/04/06)
- Internal change: Uses the caption3 kernel now

v3.0 (2003/12/20)
- Completely rewritten in cooperation with Frank Mittelbach and Steven Cochran

v3.1 (2007/09/01)
- Improved compatibility to supported document classes and packages, but decreased compatibility to non-supported document classes and packages
- Support of the AMS & SMF document classes added
- Support of the `beamer' document class added
- Support of the `KOMA-Script' document classes added
- Support of the `floatflt' package added
- Support of the `fltpage' package added
- Support of the `picinpar' package added
- Support of the `picins' package added
- Support of the `threeparttable' package added
- Support of the `wrapfig' package added
- Support of the `xtab' package added
- Check against incompatible `ftcap' package added
- Check against incompatible `nonfloat' package added
- Check against incompatible `topcapt' package added
- Does not process global options anymore to avoid conflicts with document class options
- New option compatibility=
- New options font+=, labelfont+= & textfont+=
- New options hypcap= & hypcapspace=
- New options list= and listformat=
- New option options=
- New options figurewithin= and tablewithin=
- Starred variant of option margin*= added
- Starred variant of option style*= added
- Starred variant of option type*= added
- Font options `normal', `normalcolor', `color', `normalfont' & `stretch' added
- Default position changed from `bottom' to `auto'
- New command \DeclareFloatingEnvironment resp. \DeclareCaptionType
- New command \DeclareCaptionListFormat
- New command \captionlistentry
- Starred variant of \clearcaptionsetup added
- Optional argument added to \clearcaptionsetup
- Starred variant of \ContinuedFloat added
- \captionsetup{...} inside longtables added
- \captionsetup[singleline]{...} added
- A \label before \caption will result in warning "\label before \caption ignored"
- The counters lofdepth & lotdepth are supported now
- Label formats have three arguments now
- Optional argument added to \DeclareCaptionFormat; "format=plain" removed from single-line options of default format
- Caption label format `brace' added

v3.2 (2011/07/30)
- Support of `beamer' document class improved
- Support of `magyar' babel option added
- Support of `sansmath' package added
- Support of `titletoc' package added to \DeclareCaptionType & \DeclareCaptionSubType
- Support of `tocbasic' package added to \DeclareCaptionType
- New options calcmargin=, calcmargin*=, calcwidth=, and calcwidth*=
- New option listtype= added
- New option parboxrestore=partial/full
- New options within= & without
- Option slc= as abbreviation of singlelinecheck= added
- Pre-defined text format `empty' added
- New command \captionbox
- New command \phantomcaption
- New command \setcaptiontype as replacement for \captionsetup{type=...}
- New command \setcaptionsubtype as replacement for \captionsetup{subtype}
- "Hyperref support is turned off because hyperref has stopped early" is not a warning anymore but an information instead

v3.3 (2013/01/06)
- Revised handling of continued floats and sub-captions
- New option box= and appropriate command \DeclareCaptionBox
- New option list-entry= (see also endfloat package documentation)
- Support of multiple optional arguments added to \captionsetup (see bicaption package documentation)
- Adapted to the elsarticle document class
- Adapted to the current version of memhfixc package, provided by the memoir document class
- Fixed compatibility problem with breqn and nag packages
- Corrects incorrect load order hyperref-float now (needs hyperref v6.82q or newer)
- New switch \ifsinglelinecaption for usage inside own commands added

v3.4 (2019/09/11)
- Label format `autodot' added (for usage within documents using KOMA-Script document class)
- Label format `unnumbered' added
- \ContinuedFloat renamed to \continuedfloat (since this is not a preamble command)
- \caption will always be re-defined now, unless `compatibility' is set to `true' (or an incompatible package is loaded)

v3.5 (2020/08/30)
- If a document class defines \caption@documentclass, an adaption to the caption package will be loaded as caption-<documentclass>.sto
- New commands \SetCaptionDefault, \AtCaptionPackage, and \AfterCaptionPackage for usage in document classes or document class adaptions
- Document class support re-written (using the new commands above)
- New commands \caption@switchdefault and \caption@restoredefault for usage in babel language packages
- Babel language support re-written (using the new commands above); furthermore it's independent on the load order now
- Support for the babel language option `latvian' added
- New command \DeclareCaptionSinglelinecheck
- New commands \ForEachCaptionType and \ForEachCaptionSubType
- Options "figure*" resp. "table*" will be applied additionally in "figure*" resp. "table*" environments (twocolumn mode only)
- Option and font option "hypersetup" added which expands to \hypersetup (if defined) resp. nothing (otherwise)

v3.6 (2022/02/20)
- Fallback to versions "v1", "v3.0", "v3.1", "v3.2", "v3.3", "v3.4", and "v3.5" added
- The caption-subcaption counter handling is now independent on the "position=" setting
- Option "compatibility=true" dropped in favor of "\usepackage{caption}[=v1]"
- Option "parboxrestore=partial/full" removed (was obsolete since v3.5)
- \captionsetup{margin={...,}} sets only the left margin, \captionsetup{margin={,...}} only the right one
- The font option "stretch" does not require the setspace package anymore
- New command \nextfloat to influence the (new) counter handling
- New command \DeclareCaptionPosition to declare custom postion settings
- New command \AtCaptionSingleLineCheck to add re-definitions to the single-line-check
- New command \captiontext to typeset a caption without counter increment and without list entry
- Optional argument added to \setcaptiontype (which specifies options to be applied additionally)
- New environments `captiongroup' and `captionblock'
- Adapted to the `tablefootnote' package


bicaption package
-----------------

v0.9 (2010/09/19)
- 1st published version (see also http://www.mrunix.de/forums/showthread.php?t=68312)

v1.0 (2011/09/03)
- Support for list entries added

v1.1 (2012/12/26)
- \captionmainlanguage and \selectcaptionlanguage added

v1.2 (2016/03/27)
- \DeclareLangDependantCaptionOption added

v1.3 (2020/10/25)
- Option "bi-separator" and command \DeclareBiCaptionSeparator added

v1.4 (2020/12/25)
- Support of all available caption fallback versions since "v3.2" added

v1.5 (2021/01/04)
- Support of the listings package added


ltcaption package
-----------------

v1.0 (2007/04/15)
- 1st version

v1.1 (2007/09/01)
- Adapted to the NTG document classes (Support of \CaptionLabelFont & \CaptionTextFont added)
- Adapted to the `floatrow' package by Olga Lapko
- New macro \LTcaptype
- New environment longtable*

v1.2 (2008/03/28)
- New skip \LTcapskip

v1.3 (2011/09/12)
- New macro \CaptionLabelSeparator

v1.4 (2013/06/01)
- Adapted to the memoir document class (v3.7b)


subcaption package
------------------

v1.0 (2008/03/16)
- 1st published version

v1.1 (2011/08/17)
- New caption option subrefformat=
- New command \phantomsubcaption

v1.2 (2018/05/13)
- Values `B' and `T' for the optional argument <outer-pos> added to the environments `subfigure' and `subtable'

v1.3 (2019/08/31)
- New command \subfloat for easy transition from the `subfig' package

v1.4 (2020/12/25)
- Support of all available caption fallback versions since "v3.1" added

v1.5 (2022/01/07)
- New environments subcaptiongroup and subcaptionblock
- New command \subcaptionlistentry to make an entry into the list of figures resp. tables
- New command \subcaptiontext to typeset a sub-caption without counter increment and list entry


==> Caption/README <==
==========================================================================

The `caption' package bundle
Release 2022-03-17
Copyright (C) 1994-2022 Axel Sommerfeldt (axel.sommerfeldt@f-m.fm)

License: LPPL = LaTeX Project Public Licence
Maintenance Status: maintained (by Axel Sommerfeldt)

Home page:
  https://gitlab.com/axelsommerfeldt/caption

If you need help for installation please visit:
  https://texfaq.org/FAQ-inst-miktexstar
  https://texfaq.org/FAQ-installthings
  https://texfaq.org/FAQ-privinst

If you need help using these packages please visit:
  https://latex.org/forum/
  https://topanswers.xyz/tex
  https://tex.stackexchange.com/
  https://golatex.de/               (German)
  https://texwelt.de/               (German)

If you think you may have found a bug in these packages,
or want to report a suggestion for improvement, please either visit
  https://gitlab.com/axelsommerfeldt/caption/issues
or send an e-mail to
  axel.sommerfeldt@f-m.fm

--------------------------------------------------------------------------

The `caption' package v3.6 offers customization of captions of floating
environments such `figure' and `table' and cooperates with the packages

  float, floatflt, fltpage, hyperref, hypcap, listings, longtable,
  picinpar, picins, rotating, sidecap, subfigure, supertabular,
  threeparttable, wrapfig, and xtab.

Furthermore the `floatrow', the `subcaption', and the `subfig' package
supports the `caption' package and uses its \captionsetup interface.

User Manual: caption.pdf (English)

An outdated user manual in Russian and German could be downloaded from
https://gitlab.com/axelsommerfeldt/caption/-/tree/master/doc/outdated

--------------------------------------------------------------------------

The `bicaption' package v1.5 supports typesetting of bilingual captions.

User Manual: bicaption.pdf (English)

--------------------------------------------------------------------------

The `ltcaption' package v1.4 fixes caption problems with
other-than-center aligned longtables. (solving LaTeX PR `tools/3387')

A bonus feature is the addition of the environment longtable* which does
not increment the table counter.

This package will be loaded automatically by the `caption' package,
but can be used without the caption package, too.

User Manual: ltcaption.pdf (English)

--------------------------------------------------------------------------

The `subcaption' package v1.5 supports typesetting of sub-captions
(by using the the sub-caption feature of the `caption' package).

User Manual: subcaption.pdf (English)

--------------------------------------------------------------------------

Note: The `newfloat' package was removed from this package bundle and was
uploaded to CTAN as stand-alone package.

Note: The `totalcount' package was removed from this package bundle and
was uploaded to CTAN as stand-alone package.

==========================================================================
(The pictures cat.eps & elephant.eps were taken with permission from the
 LaTeX Companion examples.)


==> Cascaras/bibliografia.tex <==
%---------------------------------------------------------------------
%
%                      configBibliografia.tex
%
%---------------------------------------------------------------------
%
% bibliografia.tex
% Copyright 2009 Marco Antonio Gomez-Martin, Pedro Pablo Gomez-Martin
%
% This file belongs to the TeXiS manual, a LaTeX template for writting
% Thesis and other documents. The complete last TeXiS package can
% be obtained from http://gaia.fdi.ucm.es/projects/texis/
%
% Although the TeXiS template itself is distributed under the 
% conditions of the LaTeX Project Public License
% (http://www.latex-project.org/lppl.txt), the manual content
% uses the CC-BY-SA license that stays that you are free:
%
%    - to share & to copy, distribute and transmit the work
%    - to remix and to adapt the work
%
% under the following conditions:
%
%    - Attribution: you must attribute the work in the manner
%      specified by the author or licensor (but not in any way that
%      suggests that they endorse you or your use of the work).
%    - Share Alike: if you alter, transform, or build upon this
%      work, you may distribute the resulting work only under the
%      same, similar or a compatible license.
%
% The complete license is available in
% http://creativecommons.org/licenses/by-sa/3.0/legalcode
%
%---------------------------------------------------------------------
%
% Fichero  que  configura  los  parámetros  de  la  generación  de  la
% bibliografía.  Existen dos  parámetros configurables:  los ficheros
% .bib que se utilizan y la frase célebre que aparece justo antes de la
% primera referencia.
%
%---------------------------------------------------------------------


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Definición de los ficheros .bib utilizados:
% \setBibFiles{<lista ficheros sin extension, separados por comas>}
% Nota:
% Es IMPORTANTE que los ficheros estén en la misma línea que
% el comando \setBibFiles. Si se desea utilizar varias líneas,
% terminarlas con una apertura de comentario.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setBibFiles{%
%nuestros, otros%
otros%
}%%
%% Creamos la bibliografia
%%
\makeBib

% Variable local para emacs, para  que encuentre el fichero maestro de
% compilación y funcionen mejor algunas teclas rápidas de AucTeX

%%%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Tesis.tex"
%%% End:

